Learning to Allocate Incentives for Incentivized Advertising via Offline Model-Based Reinforcement Learning

Complete your ad view and grab a 5-cent bonus! In incentivized advertising, a platform promises users a bonus before observing downstream ad revenue, encouraging them to click and complete ads. It must balance the incentive promised in advance against the revenue realized afterward: insufficient incentives forfeit monetization opportunities, whereas excessive incentives reduce net profit. Because current incentives may also shape user expectations and future engagement, incentive allocation is a sequential decision problem with delayed revenue, cost sensitivity, and carryover effects. Existing work has not studied decision-making algorithms for this setting. Auto-bidding assumes available ad opportunities, while targeted promotion optimizes incentives outside the ad monetization pipeline. We formulate the problem as an MDP and develop an offline model-based RL framework for cost-controllable sequential incentive allocation. It learns a world model of user feedback and ad revenue, then performs conservative policy optimization. An independent counterfactual scorer evaluates each learned policy on held-out logs, enabling pre-launch selection without costly online exposure. Experiments on large-scale industrial data and online A/B tests show that the scorer provides a stable offline signal. The deployment path from causal inference to offline RL and then Offline-MBRL further validates the framework: MB-IQL improves per-user net profit by 7.96\% over TD3+BC, whereas reverting to plain IQL reduces it by 6.56\% (both \(p<0.0001\)).

==> tables/cdp_odp_ab.tex <==
\begin{table}[t]
  \caption{This independent concurrent A/B test diagnoses delivery-pressure cost position and is not used for cross-experiment policy ranking. MAB is the online policy and TD3+BC is the candidate policy in every group; parentheses show $p$-values, and $\sim$0 denotes $p<0.0001$.}
  \label{tab:cdp_odp_ab}
  \centering
  \setlength{\tabcolsep}{2.8pt}
  \renewcommand{\arraystretch}{0.95}
  \begin{tabular}{lccc}
    \toprule
    Metric & Group 1 & Group 2 & Group 3 \\
    \midrule
    Online $\pi$ & MAB & MAB & MAB \\
    Candidate $\pi$ & TD3+BC & TD3+BC & TD3+BC \\
    \midrule
    cost/u. & $-0.9\%$ (0.9) & $+3.6\%$ (0.1) & \textbf{\textcolor{green!50!black}{+7.1\% ($\sim$0)}} \\
    % CI (\%) & [-5.1,+3.3] & [-0.6,+7.8] & [+2.9,+11.3] \\
    net p./u. & \textbf{\textcolor{green!50!black}{+9.2\% ($\sim$0)}} & \textbf{\textcolor{green!50!black}{+35.8\% ($\sim$0)}} & \textbf{\textcolor{green!50!black}{+42.5\% ($\sim$0)}} \\
    % CI (\%) & [+1.6,+16.8] & [+28.2,+43.4] & [+34.9,+50.1] \\
    \bottomrule
  \end{tabular}
\end{table}

